ChatPose: Chatting about 3D Human Pose

We introduce ChatPose, a framework employing Large Language Models (LLMs) to understand and reason about 3D human poses from images or textual descriptions. Our work is motivated by the human ability to intuitively understand postures from a single image or a brief description, a process that intertwines image interpretation, world knowledge, and an understanding of body language. Traditional human pose estimation and generation methods often operate in isolation, lacking semantic understanding and reasoning abilities. ChatPose addresses these limitations by embedding SMPL poses as distinct signal tokens within a multimodal LLM, enabling the direct generation of 3D body poses from both textual and visual inputs. Leveraging the powerful capabilities of multimodal LLMs, ChatPose unifies classical 3D human pose and generation tasks while offering user interactions. Additionally, ChatPose empowers LLMs to apply their extensive world knowledge in reasoning about human poses, leading to two advanced tasks: speculative pose generation and reasoning about pose estimation. These tasks involve reasoning about humans to generate 3D poses from subtle text queries, possibly accompanied by images. We establish benchmarks for these tasks, moving beyond traditional 3D pose generation and estimation methods. Our results show that ChatPose outperforms existing multimodal LLMs and task-specific methods on these newly proposed tasks. Furthermore, ChatPose's ability to understand and generate 3D human poses based on complex reasoning opens new directions in human pose analysis.

==> rebuttal/table_RPE_full.tex <==
\begin{table}[t]
	\centering
	\scriptsize
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{|c|c|c|c|}
			\toprule
			\multirow{2}[4]{*}{Method} & \multicolumn{2}{c|}{ SPG } & \multirow{2}[4]{*}{\makecell{RPE}}  \\
			\cmidrule(lr){2-3}
			& {$R^{P2T}$} $\uparrow$  & {$R^{P2T}$} $\downarrow$ &  \\
			\midrule
			% LLaVA crop + SPIN & - & - & 153.9/84.5/11.0 \\
			% LLaVA crop + HMR 2.0 & - & - & 132.7/75.6/10.0 \\
			% GT Crop + HMR2 2.0 & - & - & 83.1/56.8/9.1 \\
			% GT Crop + HMR2 2.0 & - & - & 83.1/56.8/9.1 \\
			% GT Crop + HMR2 2.0 & - & - & 83.1/56.8/9.1 \\
			LLaVA + PoseScript (w/o ICL) & 1.8/2.7/5.5 & 0.9/2.9/4.5  & - \\
			LLaVA + PoseScript (w/ ICL) & 1.4/2.9/4.7 & 1.5/2.9/4.7 & - \\
			GPT4 + PoseScript (w/o ICL) & 1.9/3.6/7.4 & 2.3/4.4/8.7 & - \\
			GPT4 + PoseScript (w/ ICL) & 2.6/4.2/7.4 & 2.6/4.4/7.1 & - \\
			PoseScript finetuned with SPG & 3.2/4.6/8.2 & 2.9/5.4/9.4 & - \\
			PoseGPT (ours) & 3.3/5.5/8.2 & 3.5/5.8/11.0 & 275.0/101.8/11.9
 \\ 
			\bottomrule
		\end{tabular} 
	}
  \vspace{-2mm}
	\caption{
	    Results of suggested baselines. ICL indicates ``in context learning", where we teach LLaVA and GPT4 with a few GT examples of converting our SPG text to more detailed PoseScript descriptions. 
	}
  \vspace{-8mm}
	\label{tab:rebuttal_rpe}
\end{table}


==> tables/04_backbone_ablation.tex <==
\begin{table}[t]
	\centering
	\scriptsize
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{|c|c|c|c|}
			\toprule
			\multirow{2}[4]{*}{Pretrained Model} & \multicolumn{2}{c|}{ Pose Estimation} & \multirow{2}[4]{*}{\makecell{Reasoning-based\\Pose Estimation}}  \\
			\cmidrule(lr){2-3}
			& 3DPW \cite{threedpw} & H36M \cite{human36m} &  \\
			\midrule
			LLaVA-V1.5-7B~\cite{liu2023improvedllava} & 84.5& 82.9 & 102.5 \\
			LLaVA-V1.5-13B~\cite{liu2023improvedllava} & 81.9 & 82.4 & 101.8  \\
			\bottomrule
		\end{tabular} 
	}
	\caption{
	            \cheading{Comparison of \model using different multi-modal LLM backbones} 
	            %
             PA-MPJPE (in mm) is reported; lower is better.
	}
  \vspace{-4mm}
	\label{tab:exp_backbone_ablation_main}
\end{table}

